Lipschitz Bounds and Provably Robust Training by Laplacian Smoothing

In this work we propose a graph-based learning framework to train models with provable robustness to adversarial perturbations. In contrast to regularization-based approaches, we formulate the adversarially robust learning problem as one of loss minimization with a Lipschitz constraint, and show that the saddle point of the associated Lagrangian is characterized by a Poisson equation with weighted Laplace operator. Further, the weighting for the Laplace operator is given by the Lagrange multiplier for the Lipschitz constraint, which modulates the sensitivity of the minimizer to perturbations. We then design a provably robust training scheme using graph-based discretization of the input space and a primal-dual algorithm to converge to the Lagrangian's saddle point. Our analysis establishes a novel connection between elliptic operators with constraint-enforced weighting and adversarial learning. We also study the complementary problem of improving the robustness of minimizers with a margin on their loss, formulated as a loss-constrained minimization problem of the Lipschitz constant. We propose a technique to obtain robustified minimizers, and evaluate fundamental Lipschitz lower bounds by approaching Lipschitz constant minimization via a sequence of gradient $p$-norm minimization problems. Ultimately, our results show that, for a desired nominal performance, there exists a fundamental lower bound on the sensitivity to adversarial perturbations that depends only on the loss function and the data distribution, and that improvements in robustness beyond this bound can only be made at the expense of nominal performance. Our training schemes provably achieve these bounds both under constraints on performance and~robustness.

==> setup.tex <==
We formulate adversarially robust learning as a loss minimization 
problem with a Lipschitz constraint:
\begin{align}\label{eq:adv_robust_expected_loss_min}
  \inf_{f \in \Lip(\mathbb{X} ; \mathbb{Y}) }~ 
  \underbrace{\mathbb{E}_{(x,y) \sim \sigma} \left[ \ell
  \left( f(x), y \right) \right]}_{\triangleq L_{\sigma}(f)},
  \qquad  \text{s.t.}~~\lip(f) \leq \alpha  ,
\end{align}
where $\mathbb{X} \subset \real^{\dim(\mathbb{X})}$
and~$\mathbb{Y} \subset \real^{\dim(\mathbb{Y})}$ are convex and
compact (closures of open and bounded sets) input and output (metric)
spaces,
%
$\ell: \mathbb{Y} \times \mathbb{Y} \rightarrow \realnonnegative$ a
strictly convex and Lipschitz continuous loss function,
%
$\sigma$ an absolutely continuous probability 
measure on~$\mathbb{X} \times \mathbb{Y}$ with
(absolutely continuous) marginal~$\mu$ supported on~$\mathbb{X}$
and conditional~$\pi$, 
%
$\Lip(\mathbb{X}; \mathbb{Y})$ the space of 
Lipschitz-continuous maps from~$\mathbb{X}$ to~$\mathbb{Y}$ and
$\lip(f)$ the Lipschitz constant of $f \in \Lip(\mathbb{X}; \mathbb{Y})$.
%
% \footnote{See
%  Lemma~\ref{lemma:strict_convexity_exptected_loss} in
%  Appendix~\ref{app:lemma_strict_convexity_exptected_loss}}
%


The class of problems \eqref{eq:adv_robust_expected_loss_min}
includes, for instance, the problem of image classification with a
constraint on the Lipschitz constant of the classifier (see
Section~\ref{sec: examples}).  In this case, $\mathbb{X}$ denotes the
space of images, $\mathbb{Y}$ the space of labels, and $\sigma$ the
joint probability distribution capturing the relation between images
and labels. Typically, image classification problems are solved by
training the weights of a neural network using a labeled dataset, thus
restricting the classifier to lie within the class specified by the
neural network architecture. Instead, and more generally, in
\eqref{eq:adv_robust_expected_loss_min} we do not restrict the class
of maps, which will allow us to derive novel insights and fundamental
bounds for adversarial learning. Finally, our choice of imposing a
hard constraint on the Lipschitz constant of the classifier (as
opposed to a regularization term as commonly done in adversarial
learning and distributionally robust optimization\fpmargin{Add
  references}) is required to provide hard guarantees on the
robustness of the minimizer to adversarial perturbations.

To see this, notice that adversarial perturbations \fpmargin{Add reference}
can be written as the perturbations on the joint distribution~$\sigma$
generated by a map~$T$ that perturbs the
inputs~$x \in \mathbb{X}$ while preserving the
outputs~$y \in \mathbb{Y}$. In compact form, the class of adversarial
perturbations can be written as:
\begin{align*}
  \mathcal{T} = \left \lbrace T 
  \; \left| \; T(x,y) = (T_1(x,y) \; , \; y),~ \text{s.t.}~~T_1(x,y)
  \in B_{\delta}(x) \cap \mathbb{X} \right. \right \rbrace,
\end{align*}
where~$B_{\delta}(x)$ is the open ball in~$\real^{\dim(\mathbb{X})}$
of radius~$\delta > 0$ and centered at~$x$. Define the sensitivity as
the worst-case increase of the loss functional following an
adversarial perturbation. That is, the sensitivity of the loss~$L$
at~$\sigma$ (and a given~$f$) is the~$L^{\infty}$-norm (with respect
to the measure~$\sigma$) of the
gradient~$\nabla_1 \ell \cdot \nabla f$ (precisely,
$\| | \nabla_1 \ell \cdot \nabla f | \|_{L^{\infty}(\mathbb{X} \times
  \mathbb{Y}, \sigma)}$).\footnote{We use $\nabla_1 \ell$ to denote
  the gradient of $\ell$ with respect to its first argument.} Notice
that
\begin{align}\label{eq: inequality derivative Lipschitz}
  \underbrace{\| | \nabla_1 \ell \cdot \nabla f | \|_{L^{\infty}(\mathbb{X} \times
  \mathbb{Y}, \sigma)}}_{\text{sensitivity of $L$ to adv. perturbation}} \leq \underbrace{\| | \nabla_1 \ell |
  \|_{L^{\infty}(\mathbb{X} \times \mathbb{Y},
  \sigma)}}_{\text{Lipschitz constant of $\ell$}}  \cdot
  \underbrace{\| | \nabla f | \|_{L^{\infty}(\mathbb{X},
  \mu)}}_{\text{Lipschitz constant of $f$}}
\end{align}
where $\mu$ is the marginal of~$\sigma$ over~$\mathbb{X}$, and
$\| | \nabla f | \|_{L^{\infty}(\mathbb{X}, \mu)}$ is the Lipschitz
constant of~$f$ over the support of~$\mu$. Thus, restricting the
search space to the class of Lipschitz maps with a
bound~$\alpha \geq 0$ on the Lipschitz constant, as in the
minimization problem~\eqref{eq:adv_robust_expected_loss_min}, is
convenient for the analysis, does not restrict the generality, and it
allows us to obtain provably robust minimizers of the loss~$L$.

%\bigskip
%\bigskip
%---------------------------
%{\color{blue}Vishaal's version}
%---------------------------
%\begin{align}
%	\min_{f \in \mathcal{F}}~ L(\sigma, f) \triangleq \mathbb{E}_{(x,y) \sim \sigma} \left[ \ell \left( f(x), y \right) \right],
%	\label{eq:expected_loss_min}
%\end{align}
%where~$\mathbb{X} \subset \real^{\dim(\mathbb{X})}$ 
%and~$\mathbb{Y} \subset \real^{\dim(\mathbb{Y})}$
%are convex and compact (closures of open and bounded sets)
%input and output (metric) spaces,
%%
%$\mathcal{F}$ is a (convex and closed) class of maps from~$\mathbb{X}$ to~$\mathbb{Y}$
%% 
%and~$\sigma \in \mathcal{P} \left( \mathbb{X} \times \mathbb{Y} \right)$
%is a joint probability measure on~$\mathbb{X} \times \mathbb{Y}$,
%with a Lipschitz continuous, strictly convex loss function~$\ell: \mathbb{Y} \times \mathbb{Y}
%\rightarrow \realnonnegative$.
%%
%We assume that~$\sigma \in \mathcal{P}(\mathbb{X} \times \mathbb{Y})$ 
%is absolutely continuous and that its marginal~$\mu \in \mathcal{P}(\mathbb{X})$
%is supported over~$\mathbb{X}$, i.e., $\supp(\mu) = \mathbb{X}$.
%
%The following lemma (proved in Appendix~\ref{app:proof_lemma_strict_convexity_exptected_loss}) 
%establishes that strict convexity of the loss function~$\ell$ induces strict convexity on
%the loss~$L(\sigma \; , \; \cdot~)$:
%%
%\begin{lemma}[Strict convexity of loss]
%\label{lemma:strict_convexity_exptected_loss}
%The loss~$L(\sigma \; , \; \cdot~)$ in~\eqref{eq:expected_loss_min} 
%is strictly convex for any~$\sigma \in \mathcal{P}(\mathbb{X} \times \mathbb{Y})$.
%\end{lemma}
%%
%%\textbf{Lipschitz constant and sensitivity to adversarial perturbations}
%%
%We consider a class of perturbations on the joint distribution~$\sigma$
%generated by a class of maps~$\mathcal{T}$ that perturb 
%the inputs~$x \in \mathbb{X}$ while preserving 
%the outputs~$y \in \mathbb{Y}$:
%%
%%[perturb the images while preserving the class labels]:
%%
%\begin{align*}
%	\mathcal{T} = \left \lbrace T 
%%\in \mathcal{B} \left(\mathbb{X} \times \mathbb{Y}; \real^{\dim(\mathbb{X})} \times \real^{\dim(\mathbb{Y})} \right) 
%\; \left| \; T(x,y) = (T_1(x,y) \; , \; y),~ \text{s.t.}~~T_1(x,y) \in B_{\delta}(x) \cap \mathbb{X} \right. \right \rbrace,
%\end{align*}
%where~$B_{\delta}(x)$ is the open ball in~$\real^{\dim(\mathbb{X})}$ of radius~$\delta > 0$, 
%centered at~$x$.
%%
%The following lemma characterizes an upper bound on perturbations 
%of the loss~$L(\; \cdot \; , \; f)$ by the class~$\mathcal{T}$ 
%and the derivative of~$L(\; \cdot \; , \; f)$
%along the tangent space of~$T \in \mathcal{T}$, for a Lipschitz map~$f$:
%%
%\begin{lemma}[Perturbation bound and derivative of loss]
%For any~$f \in \Lip(\mathbb{X}; \mathbb{Y})$ and~$T \in \mathcal{T}$,
%we have:
%\begin{align*}
%	\left| L(T_{\#}\sigma , f) - L(\sigma, f) \right| \leq \lip(\ell) \lip(f) \delta.
%\end{align*}
%Moreover, the derivative of the loss~$L(\; \cdot \; , \; f) : \mathcal{P}(\mathbb{X} \times \mathbb{Y}) \rightarrow \realnonnegative$ 
%at~$\sigma \in \mathcal{P}(\mathbb{X} \times \mathbb{Y})$, along the tangent space of~$\mathcal{T}$, is given by:
%\begin{align*}
%	D_{T} L(\sigma, f) = \mathbb{E}_{(x,y) \sim \sigma} \left[ \left \langle \nabla_1\ell (f(x), y) \cdot \nabla f(x) \; , \; T_1(x,y) \right \rangle \right].
%\end{align*}
%%
%\end{lemma}
%%
%The proof of Lemma~\ref{lemma:loss_derivative_adversarial} can be
%found in Appendix~\ref{app:proof_lemma_los_derivative_adversarial}.
%%
%From Lemma~\ref{lemma:loss_derivative_adversarial}, we infer that
%the sensitivity of the loss~$L$ at~$\sigma$ (and a given~$f$) to 
%adversarial perturbations is modulated by the gradient~$\nabla_1 \ell \cdot \nabla f$.
%We therefore define the sensitivity of the loss~$L$ at~$\sigma$ (and a given~$f$) 
%to be the~$L^{\infty}$-norm (w.r.t. the measure~$\sigma$) of the gradient~$\nabla_1 \ell \cdot \nabla f$,
%i.e.,~$\| | \nabla_1 \ell \cdot \nabla f | \|_{L^{\infty}(\mathbb{X} \times \mathbb{Y}, \sigma)}$.
%%
%Moreover, we have the bound $\| | \nabla_1 \ell \cdot \nabla f | \|_{L^{\infty}(\mathbb{X} \times \mathbb{Y}, \sigma)}
%\leq \| | \nabla_1 \ell | \|_{L^{\infty}(\mathbb{X} \times \mathbb{Y}, \sigma)} \cdot 
%\| | \nabla f | \|_{L^{\infty}(\mathbb{X}, \mu)}$, where~$\mu \in \mathcal{P}(\mathbb{X})$ 
%is the marginal over~$\mathbb{X}$ of~$\sigma$.
%%
%We note that~$\| | \nabla f | \|_{L^{\infty}(\mathbb{X}, \mu)}$ is the Lipschitz
%constant of~$f$ over the support of~$\mu$.
%
%The adversarially robust loss minimization problem is therefore given by:
%\begin{align}
%		\inf_{f \in \Lip(\mathbb{X}, \mu) }~ \left \lbrace L(\sigma, f) 	\qquad  \text{s.t.}~~\lip(f) \leq \alpha \right \rbrace.
%		\label{eq:adv_robust_expected_loss_min}
%\end{align}
%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End: 
